LSVOS Challenge Report: Large-scale Complex and Long Video Object Segmentation

Despite the promising performance of current video segmentation models on existing benchmarks, these models still struggle with complex scenes. In this paper, we introduce the 6th Large-scale Video Object Segmentation (LSVOS) challenge in conjunction with ECCV 2024 workshop. This year's challenge includes two tasks: Video Object Segmentation (VOS) and Referring Video Object Segmentation (RVOS). In this year, we replace the classic YouTube-VOS and YouTube-RVOS benchmark with latest datasets MOSE, LVOS, and MeViS to assess VOS under more challenging complex environments. This year's challenge attracted 129 registered teams from more than 20 institutes across over 8 countries. This report include the challenge and dataset introduction, and the methods used by top 7 teams in two tracks. More details can be found in our homepage https://lsvos.github.io/.

==> sections/2_related.tex <==
\section{Related Works}
Video object segmentation (VOS) focuses on segmenting a specific object across the entire sequence of a video. Depending on how the target object is identified, VOS can be categorized into four primary settings: \ie, semi-supervised VOS (or semi-automatic VOS~\cite{zhou2022survey} or one-shot VOS), unsupervised VOS (or automatic VOS~\cite{zhou2022survey} or zero-shot VOS), interactive VOS, and referring VOS. Each of these settings differs in the level of human intervention required and the method used to delineate the target object.

\subsection{Semi-supervised VOS} 
Semi-supervised video object segmentation (or one-shot video object segmentation)~\cite{caelles2017one} aims to track and segment the target object across the subsequent video frames based on the given object mask in the first frame. Most existing approaches can be categorized into propagation-based methods and matching-based methods. Propagation-based methods~\cite{DBLP:conf/cvpr/PerazziKBSS17,jang2017online,DBLP:conf/cvpr/JampaniGG17,xiao2018monet,hu2018motion,han2018reinforcement,youtube_vos,cheng2018fast,xu2019mhp,chen2020state,huang2020fast,wug2018fast,lin2019agss,zhang2019fast} guide the mask generation for the current frame using the mask from the previous frame, effectively propagating target object information frame by frame. In contrast, matching-based methods~\cite{DBLP:conf/iccv/YoonRKLSK17,cheng2018fast,voigtlaender2019feelvos,wang2019ranet,Duarte_2019_ICCV,Oh_2019_ICCV,hong2024onetracker,zhang2020transductive,yang2020collaborative,li2024onevos,Hu_2021_CVPR,yan2023panovos，duke2021sstvos} store an embedding of the target object and perform per-pixel classification to determine the similarity between each pixel's feature and the stored embedding of the target object.


\subsection{Referring VOS} 
Referring video object segmentation~\cite{seo2020urvos, liu2022instance, wang2019asymmetric, Ding_2022_CVPR,phraseclick,ye2021referring,ding2021vision,VLT} is an emerging task within the field of video object segmentation that integrates multi-modal information. In Referring VOS, a natural language expression is provided to specify the target object, with the goal of segmenting that object consistently throughout the entire video sequence. Current referring video object segmentation methods can be be broadly classified into two categories: bottom-up methods and top-down approaches. Bottom-up methods~\cite{seo2020urvos, VLTPAMI, fang2023instructseq，liu2021cmpc} typically involve segmenting the target object in the first frame and then propagating the generated mask across subsequent frames, or alternatively, performing independent image segmentation on each frame followed by associating these segmented masks across the video. Top-down methods~\cite{liang2021topdown, Botach_2022_CVPR, Wu_2022_CVPR} adopt a more exhaustive strategy by proposing all potential tracklets within the video and then selecting the one which best matches the given language expression as the final output.





